Heavy-quark production in deep-inelastic scattering -- Mellin moments of structure functions

We compute Mellin moments of the heavy-quark structure functions in deep-inelastic scattering at next-to-leading order in quantum chromodynamics, retaining their full dependence on the heavy-quark mass. Using the optical theorem and the operator product expansion, we derive analytic results for fixed Mellin moments $N = 2$ to $22$ of the structure functions $F_2$ and $F_L$. Our results reproduce the known expressions in the relevant asymptotic limits, in particular for virtualities of the exchanged photon $Q^2$ much larger than the heavy-quark mass squared $m^2$, and are in agreement with existing parametrisations of the next-to-leading-order coefficient functions. The computational set-up developed in this work also provides a direct pathway toward extending these calculations to next-to-next-to-leading order.

==> hq-merged/commands.tex <==
\newcommand{\LineNoNumber}{\\ \nonumber}
\newcommand{\LineNumber}{\\}

\newcommand{\GeV}{\text{GeV}}

\newcommand{\scalar}{\text{s}}
\renewcommand{\vector}{\text{v}}
\newcommand{\axial}{\text{a}}
\newcommand{\light}{\text{l}}
\newcommand{\heavy}{\text{h}}
\newcommand{\flavour}{\text{f}}
\newcommand{\parton}{\text{p}}

\newcommand{\ren}{\text{ren}}
\newcommand{\const}{\text{const}}

\newcommand{\ps}{\text{ps}}
\newcommand{\ns}{\text{ns}}

\newcommand{\gammafive}{\gamma_5}

\newcommand{\comma}{\, ,}
\newcommand{\period}{\, .}

\RenewDocumentCommand{\sp}{O{}mm}{
  \ifthenelse{\equal{#2}{#3}}
    {\def\spresult{#2^2}}
    {\def\spresult{#2 \cdot #3}}
  \ifthenelse{\equal{#1}{}}
    {\ensuremath{\spresult}}
    {\ensuremath{\left( \spresult \right)^{#1}}}
}

\newcommand{\bjorken}{x}

\newcommand{\intn}[2]{\int \dd[#2]{#1}}
\NewDocumentCommand{\integral}{m m m}{\int_{#2}^{#3} \dd{#1}}

\newcommand{\disc}{\text{Disc}}

\NewDocumentCommand{\vectors}{o m m m m}{%
  \IfNoValueTF{#1}
    {\tensor{#2}{#3{\lambda_{#4}}} \dots \tensor{#2}{#3{\lambda_{#5}}}}%
    {\tensor{#2}{#3{\{ \lambda_{#4}}} \dots \tensor{#2}{#3{\lambda_{#5}\} }} }%
}

\newcommand{\psq}{\text{q}}
\newcommand{\psc}{\text{c}}
\newcommand{\psg}{\text{g}}

\NewDocumentCommand{\coef}{m m O{}}{%
  C^{#1}_{#2\IfNoValueTF{#3}{}{,#3}}%
}

\newcommand{\mzv}[1]{\zeta_{#1}}

\newcommand{\poly}[3]{\text{P}_{{#1},{#2},{#3}}}
\newcommand{\num}[4][]
  {\text{P}_{#2,#3,#4}^{#1}}

\newcommand{\hpl}[1]{\text{H}_{#1}}

\renewcommand{\order}[1]{\mathcal{O}\left(#1\right)}

\NewDocumentCommand{\ome}{m m O{}}{%
  A^{#1}_{#2\IfNoValueTF{#3}{}{,#3}}%
}

\newcommand{\weinbergangle}{\theta_\text{W}}

\newcommand{\gammaf}[1]{\Gamma\left(#1\right)}
\newcommand{\poch}[2]{\left(#1\right)_{#2}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceiling}[1]{\lceil #1 \rceil}

\newcommand{\as}{\alpha_s}
\newcommand{\ep}{\epsilon}

\newcommand{\adim}[2]{\gamma_{\text{#1}}^{(#2)}}
\newcommand{\cfun}[4]{c_{\text{#1},\text{#2}}^{(#3,#4)}}
\newcommand{\Cfun}[2]{C_{\text{#1},\text{#2}}}
\newcommand{\Tfun}[2]{T_{\text{#1},\text{#2}}}
\newcommand{\bfun}[1]{\beta_{#1}}

\newcommand{\boson}[1]{\text{b}_{#1}}

\newcommand{\cmom}[4]{c^{N,(#3,#4)}_{#1,#2}}
\renewcommand{\bfun}[1]{\beta_{#1}}
\renewcommand{\adim}[3]{\gamma^{N,(#3)}_{#1#2}}
\newtheorem*{lemma*}{Lemma}


==> hq-merged/tables/numerics.tex <==
\renewcommand{\arraystretch}{1.1} % double spacing in table
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\begin{longtable}{@{\extracolsep{\fill}}|c|c|c|c|c|@{}}
\hline 
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,q}^{N,(2,0)}$} &
\multicolumn{2}{c|}{$c_{2,q}^{N,(2,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endfirsthead

\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,q}^{N,(2,0)}$} &
\multicolumn{2}{c|}{$c_{2,q}^{N,(2,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endhead

2 & $-2.663968441e-01$ & $-2.6599e-01$ & $-1.819031902e+00$ & $-1.8187e+00$ \\
4 & $-2.291865727e-02$ & $-2.2898e-02$ & $-1.440499763e-01$ & $-1.4401e-01$ \\
6 & $-3.037959700e-03$ & $-3.0392e-03$ & $-2.040592390e-02$ & $-2.0418e-02$ \\
8 & $-5.184054510e-04$ & $-5.1947e-04$ & $-3.811432361e-03$ & $-3.8175e-03$ \\
10 & $-1.027971471e-04$ & $-1.0318e-04$ & $-8.290910647e-04$ & $-8.3117e-04$ \\
12 & $-2.252325062e-05$ & $-2.2641e-05$ & $-1.985751721e-04$ & $-1.9923e-04$ \\
14 & $-5.299818794e-06$ & $-5.3350e-06$ & $-5.082020292e-05$ & $-5.1024e-05$ \\
16 & $-1.315786777e-06$ & $-1.3262e-06$ & $-1.365120445e-05$ & $-1.3714e-05$ \\
18 & $-3.406331187e-07$ & $-3.4374e-07$ & $-3.804753682e-06$ & $-3.8243e-06$ \\
20 & $-9.119679388e-08$ & $-9.2130e-08$ & $-1.091674299e-06$ & $-1.0978e-06$ \\
22 & $-2.509868611e-08$ & $-2.5381e-08$ & $-3.206582357e-07$ & $-3.2258e-07$ \\
\hline
\caption{Comparison of the numerical values of the singlet coefficient function moments at NLO, 
cf.~Eq.(\ref{eq:def-coeffs}), 
for $m = 2 \sqrt{2}\, \text{GeV}$ and $Q = 7\, \text{GeV}$ such that $\kappa = 8 /49$, for the scale choice $\mu_r=\mu_f=Q$.
}
\label{tab:C2qPS} \\
\end{longtable}

\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\begin{longtable}{@{\extracolsep{\fill}}|c|c|c|c|c|@{}}
\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,q}^{N,\text{NS},(2,0)}$} &
\multicolumn{2}{c|}{$c_{2,q}^{N,\text{NS},(2,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endfirsthead

\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,q}^{N,\text{NS},(2,0)}$} &
\multicolumn{2}{c|}{$c_{2,q}^{N,\text{NS},(2,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endhead

2 & $1.269706065e-01$ & $1.2691e-01$ & $3.828697684e-01$ & $3.8268e-01$ \\
4 & $7.773989042e-03$ & $7.7697e-03$ & $1.899084702e-02$ & $1.8981e-02$ \\
6 & $8.451385732e-04$ & $8.4611e-04$ & $1.953555304e-03$ & $1.9556e-03$ \\
8 & $1.218724089e-04$ & $1.2232e-04$ & $2.757969313e-04$ & $2.7672e-04$ \\
10 & $2.086984108e-05$ & $2.1002e-05$ & $4.678690020e-05$ & $4.7059e-05$ \\
12 & $4.015640039e-06$ & $4.0518e-06$ & $8.963806878e-06$ & $9.0378e-06$ \\
14 & $8.409051715e-07$ & $8.5059e-07$ & $1.873670645e-06$ & $1.8935e-06$ \\
16 & $1.878096423e-07$ & $1.9041e-07$ & $4.182500377e-07$ & $4.2360e-07$ \\
18 & $4.413049803e-08$ & $4.4839e-08$ & $9.829615433e-08$ & $9.9755e-08$ \\
20 & $1.080458841e-08$ & $1.1000e-08$ & $2.408000184e-08$ & $2.4483e-08$ \\
22 & $2.736748775e-09$ & $2.7912e-09$ & $6.104188218e-09$ & $6.2172e-09$ \\
\hline
\caption{
Same as \autoref{tab:C2qPS} for the non-singlet coefficient function moments at NLO. The values for $c_{2,q}^{N,\text{NS},(2,0)}$ in column 3 (KMS) 
are subject to the subtraction in Eq.~(\ref{eq:F2ns-subtract}).
}
\label{tab:C2qNS}\\
\end{longtable}

\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\begin{longtable}{@{\extracolsep{\fill}}|c|c|c|c|c|@{}}
\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,g}^{N,(1,0)}$} &
\multicolumn{2}{c|}{$c_{2,g}^{N,(1,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endfirsthead

\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,g}^{N,(1,0)}$} &
\multicolumn{2}{c|}{$c_{2,g}^{N,(1,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endhead

2 & $8.867283709e-02$ & $8.8673e-02$ & $5.028907767e-01$ & $5.0289e-01$ \\
4 & $1.103046457e-02$ & $1.1030e-02$ & $6.175564320e-02$ & $6.1756e-02$ \\
6 & $1.917444241e-03$ & $1.9174e-03$ & $1.183561754e-02$ & $1.1836e-02$ \\
8 & $3.966816131e-04$ & $3.9668e-04$ & $2.731109006e-03$ & $2.7311e-03$ \\
10 & $9.137167103e-05$ & $9.1372e-05$ & $6.987846232e-04$ & $6.9878e-04$ \\
12 & $2.264262570e-05$ & $2.2643e-05$ & $1.909719930e-04$ & $1.9097e-04$ \\
14 & $5.916619363e-06$ & $5.9166e-06$ & $5.463077020e-05$ & $5.4631e-05$ \\
16 & $1.609557695e-06$ & $1.6096e-06$ & $1.616052219e-05$ & $1.6161e-05$ \\
18 & $4.519332213e-07$ & $4.5193e-07$ & $4.904449068e-06$ & $4.9044e-06$ \\
20 & $1.301724905e-07$ & $1.3017e-07$ & $1.518757609e-06$ & $1.5188e-06$ \\
22 & $3.829032869e-08$ & $3.8290e-08$ & $4.780440303e-07$ & $4.7804e-07$ \\
\hline
\caption{
Same as \autoref{tab:C2qPS} for the gluon coefficient function moments at leading order.
}
\label{tab:C1g}\\
\end{longtable}

\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\begin{longtable}{@{\extracolsep{\fill}}|c|c|c|c|c|@{}}
\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,g}^{N,(2,0)}$} &
\multicolumn{2}{c|}{$c_{2,g}^{N,(2,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endfirsthead

\hline
\multicolumn{1}{|c|}{} &
\multicolumn{2}{c|}{$c_{L,g}^{N,(2,0)}$} &
\multicolumn{2}{c|}{$c_{2,g}^{N,(2,0)}$} \\
\hline
$N$ & KMS & RSvN & KMS & RSvN \\
\hline
\hline
\endhead

2 & $3.378659570e+00$ & $3.4037e+00$ & $1.606527957e+01$ & $1.6121e+01$ \\
4 & $7.289865120e-01$ & $7.3158e-01$ & $3.680483878e+00$ & $3.6872e+00$ \\
6 & $1.676777828e-01$ & $1.6809e-01$ & $9.457069517e-01$ & $9.4677e-01$ \\
8 & $4.148549496e-02$ & $4.1576e-02$ & $2.623839998e-01$ & $2.6259e-01$ \\
10 & $1.087276123e-02$ & $1.0897e-02$ & $7.663126763e-02$ & $7.6681e-02$ \\
12 & $2.977571974e-03$ & $2.9849e-03$ & $2.319720217e-02$ & $2.3211e-02$ \\
14 & $8.436717814e-04$ & $8.4599e-04$ & $7.208613114e-03$ & $7.2126e-03$ \\
16 & $2.455922015e-04$ & $2.4633e-04$ & $2.285220881e-03$ & $2.2865e-03$ \\
18 & $7.307379587e-05$ & $7.3315e-05$ & $7.358664768e-04$ & $7.3627e-04$ \\
20 & $2.213903270e-05$ & $2.2218e-05$ & $2.399582635e-04$ & $2.4009e-04$ \\
22 & $6.809936693e-06$ & $6.8358e-06$ & $7.906076590e-05$ & $7.9104e-05$ \\
\hline
\caption{
Same as \autoref{tab:C2qPS} for the gluon coefficient function moments at NLO.
} 
\label{tab:C2g}\\
\end{longtable}


